MetaWeather: Few-Shot Weather-Degraded Image Restoration

Real-world weather conditions are intricate and often occur concurrently. However, most existing restoration approaches are limited in their applicability to specific weather conditions in training data and struggle to generalize to unseen weather types, including real-world weather conditions. To address this issue, we introduce MetaWeather, a universal approach that can handle diverse and novel weather conditions with a single unified model. Extending a powerful meta-learning framework, MetaWeather formulates the task of weather-degraded image restoration as a few-shot adaptation problem that predicts the degradation pattern of a query image, and learns to adapt to unseen weather conditions through a novel spatial-channel matching algorithm. Experimental results on the BID Task II.A, SPA-Data, and RealSnow datasets demonstrate that the proposed method can adapt to unseen weather conditions, significantly outperforming the state-of-the-art multi-weather image restoration methods.

==> table/ablation_dpmm.tex <==
\begin{table*}[h!]
\centering
\def\arraystretch{1.25}
\resizebox{1.0\columnwidth}{!}{
{\small
% \setlength{\tabcolsep}{1.75pt}
\begin{tabular}{cc|cc|cc|cc|cc|cc||cc}
\hline
\toprule
\normalfont{ } 
\multirow{2}{*}{\shortstack{Spatial\\\;\; Matching \;\;}} & \multirow{2}{*}{\shortstack{Channel\\\;\; Matching \;\;}}  & \multicolumn{2}{c|}{$\text{R+S}$} & \multicolumn{2}{c|}{$\text{R+H}_L$} & \multicolumn{2}{c|}{$\text{R+H}_H$} & \multicolumn{2}{c|}{R+D+$H_M$} & \multicolumn{2}{c||}{R+D+S+$H_M$}  & \multicolumn{2}{c}{Average}\\
% \hline
\multirow{2}{*}{} & \multirow{2}{*} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM  & PSNR & SSIM & PSNR & SSIM\\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
- & - & 27.66 & 0.8516 & 25.54 & 0.8651 & 21.12 & 0.7858 & 22.45 & 0.7847 & 21.29 & 0.7320 & 23.61 & 0.8038\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\checkmark & - &  27.46 & 0.8413 & 24.94 & 0.8676 & 21.63 & 0.7958 & 22.44 & 0.7959 & 21.33 & 0.7321 & 23.56 & 0.8065\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
- & \checkmark &  \textbf{28.61} & \underline{0.8726} & \underline{25.75} & \underline{0.8849} & \textbf{22.74} & \textbf{0.8340} & \underline{22.60} & \underline{0.8127} & \underline{22.07} & \underline{0.7697} & \underline{24.35} & \underline{0.8348}\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\checkmark & \checkmark & \underline{28.54} & \textbf{0.8728} & \textbf{25.77} & \textbf{0.8876} & \underline{22.58} & \underline{0.8281} & \textbf{22.80} & \textbf{0.8188} & \textbf{22.16} & \textbf{0.7775} & \textbf{24.37} & \textbf{0.8370}\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bottomrule
\end{tabular}
}
}
\caption{Ablation study on components of DPMM. The \textbf{best} results are highlighted. The ablation study on the value of $k$ can be found in the supplementary material.}
\label{tab:ablation_table}
\end{table*}

==> table/main_table.tex <==

\begin{table*}[t!]
\centering
\def\arraystretch{1.25}
\resizebox{1.0\columnwidth}{!}{
{\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{c|cc|cc|cc|cc|cc||cc}
\hline
\toprule
\normalfont{ } 
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{$\text{R+S}$} & \multicolumn{2}{c|}{$\text{R+H}_L$} & \multicolumn{2}{c|}{$\text{R+H}_H$} & \multicolumn{2}{c|}{R+D+H$_M$} & \multicolumn{2}{c||}{R+D+S+H$_M$}  & \multicolumn{2}{c}{Average}\\
% \hline
\multirow{2}{*}{} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM  & PSNR & SSIM & PSNR & SSIM\\
\hline
TransWeather~\cite{valanarasu2022transweather} & 25.82 & 0.8056 & 24.68 & 0.8484 & \underline{21.48} & 0.7770 & \underline{21.71} & 0.7569 & 20.72 & 0.6900 & \underline{22.88} & 0.7756\\
AirNet~\cite{li2022all}  & 26.63 & 0.8206 & 23.43 & 0.8535 & 17.35 & 0.7260 & 18.06 & 0.7130 & 17.97 & 0.6493 & 20.69 & 0.7525\\
NAFNet~\cite{chen2022simple} & 26.45 & 0.8428 & 24.96 & 0.8724 & 20.91 & 0.7808 & 21.29 & 0.7751 & 19.52 & 0.7001 & 22.63 & 0.7942\\
Restormer~\cite{zamir2022restormer} & 27.73 & \textbf{0.8773} & \underline{25.14} & 0.8791 & 20.75 & 0.7905 & 21.21 & \underline{0.7871} & 18.52 & 0.7311 & 22.67 & \underline{0.8130}\\
FocalNet~\cite{cui2023focal} & 26.58 & 0.8358 & 24.51 & 0.8636 & 20.16 & 0.7677 & 20.62 & 0.7599 & 18.79 & 0.6909 & 22.13 & 0.7836\\
MPRNet~\cite{zamir2021multi} & \underline{27.98} & 0.8655 & 24.70 & \underline{0.8849} & 20.44 & \underline{0.8008} & 19.81 & 0.7725 & \underline{20.94} & \underline{0.7390} & 22.77 & 0.8125\\ 
MAXIM~\cite{tu2022maxim} & - \\
 % DT & -\\
 % Diffusion(TBD) & -\\
\hline
%MetaWeather-C & 16.10 & 28.61 & 0.8726 & 25.75 & 0.8849 & 22.74 & 0.8340 & 22.60 & 0.8127 & 22.07 & 0.7697 & 24.35 & 0.8348 \\ 
Ours & \textbf{28.54} & \underline{0.8728} & \textbf{25.77} & \textbf{0.8876} & \textbf{22.58} & \textbf{0.8281} & \textbf{22.80} & \textbf{0.8188} & \textbf{22.16} & \textbf{0.7775} & \textbf{24.37} & \textbf{0.8370}\\ 
\bottomrule
\end{tabular}
}
}
\caption{Quantitative comparison on BID Task \RNum{2}.A dataset~\cite{han2022blind}. All models are adapted with a 2-shot support set for each case. 
% Results are ordered by PSNR. 
The \textbf{best} and \underline{second-best} results are highlighted.}
% Note that each case consists of (1) rain streak; (2) rain streak + snow; (3) rain streak + light haze; (4) rain streak + heavy haze; (5) rain streak + moderate haze + raindrop; (6) rain streak + snow + moderate haze + raindrop.}
% \vspace{-11pt}
\label{tab:main_table}
\end{table*}

==> table/supp_VTM.tex <==
\begin{table}[hb]
\caption{Quantitative comparison with VTM~\cite{kim2023universal} on the BID Task \RNum{2}.A ~\cite{han2022blind}, SPA-Data~\cite{Wang2019spa} and RealSnow~\cite{zhu2023learning} datasets. The \textbf{best} results are highlighted.}

\begin{subtable}[h]{\textwidth}
\centering
\def\arraystretch{1.3}
{
% \setlength{\tabcolsep}{0.2pt}
\caption{\small Co-occuring weather types~\cite{han2022blind}}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc||cc}
\hline
\toprule
\multirow{2}{*}{Method}  & \multicolumn{2}{c|}{$\text{R+S}$} & \multicolumn{2}{c|}{$\text{R+H}_\text{L}$} & \multicolumn{2}{c|}{$\text{R+H}_\text{H}$} & \multicolumn{2}{c|}{R+D+H$_\text{M}$} & \multicolumn{2}{c||}{R+D+S+H$_\text{M}$}  & \multicolumn{2}{c}{Average}\\
% \hline
\multirow{2}{*}{} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM  & PSNR & SSIM & PSNR & SSIM\\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
VTM~\cite{kim2023universal} & 26.99 & 0.8275 & 24.15 & 0.8310 & 19.15 & 0.7309 & 20.65 & 0.7388 & 20.03 & 0.6821 & 22.19 & 0.7621\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{MetaWeather} &  \textbf{27.88} & \textbf{0.8574} & \textbf{25.85} & \textbf{0.8790} & \textbf{22.02} & \textbf{0.8137} & \textbf{23.24} & \textbf{0.8142} & \textbf{22.42} & \textbf{0.7575} & \textbf{24.28} & \textbf{0.8244}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bottomrule
\end{tabular}
}
}

% The \textbf{best} results are highlighted. The ablation study on the value of $k$ can be found in the supplementary material.}
\label{tab:vtm_bid}
\end{subtable}

\vspace{1em}

\begin{subtable}[hb]{\textwidth}
\centering
\caption{\small Real-world conditions}

\def\arraystretch{1.2}
\resizebox{0.6\columnwidth}{!}
{
{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{c|cc|cc}
\hline
\toprule
\normalfont{ } 
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{SPA-Data~\cite{wang2019panet}}  & \multicolumn{2}{c}{RealSnow\cite{zhu2023learning}}\\
% \hline
 & PSNR & SSIM & PSNR & SSIM\\
\hline
VTM~\cite{kim2023universal} & 32.27 & 0.9151 & 28.87 & 0.9099\\

\textbf{MetaWeather} & \textbf{34.81} & \textbf{0.9394} & \textbf{30.15} & \textbf{0.9222}\\
\bottomrule
\end{tabular}
}
}
% \vspace{-11pt}
\label{tab:vtm_real}
\end{subtable}

\label{tab:vtm}
\end{table}

==> table/supp_pretrain.tex <==
\begin{table}[b]
\centering
\caption{Ablation study on pretrain knowledge. The \textbf{best} results are highlighted.}
\def\arraystretch{1.3}
{
% \setlength{\tabcolsep}{0.2pt}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc||cc}
\hline
\toprule
\multirow{2}{*}{Method}  & \multicolumn{2}{c|}{$\text{R+S}$} & \multicolumn{2}{c|}{$\text{R+H}_\text{L}$} & \multicolumn{2}{c|}{$\text{R+H}_\text{H}$} & \multicolumn{2}{c|}{R+D+H$_\text{M}$} & \multicolumn{2}{c||}{R+D+S+H$_\text{M}$}  & \multicolumn{2}{c}{Average}\\
% \hline
\multirow{2}{*}{} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM  & PSNR & SSIM & PSNR & SSIM\\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
w/o SimMIM~\cite{xie2022simmim} & 25.31 & 0.7812 & 22.63 & 0.8110 & 19.20 & 0.6972 & 17.50 & 0.6816 & 17.37 & 0.6039 & 20.40 & 0.7150\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
w/ SimMIM~\cite{xie2022simmim} &  \textbf{27.88} & \textbf{0.8574} & \textbf{25.85} & \textbf{0.8790} & \textbf{22.02} & \textbf{0.8137} & \textbf{23.24} & \textbf{0.8142} & \textbf{22.42} & \textbf{0.7575} & \textbf{24.28} & \textbf{0.8244}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bottomrule
\end{tabular}
}
}

% The \textbf{best} results are highlighted. The ablation study on the value of $k$ can be found in the supplementary material.}
\label{tab:contents}
\end{table}

==> table/supp_sidd.tex <==

\begin{table*}[t!]
\centering
\caption{Quantitative comparison with VTM~\cite{kim2023universal} on the SIDD~\cite{abdelhamed2018high} dataset. The \textbf{best} results are highlighted.}
\def\arraystretch{1.15}
\resizebox{0.5\columnwidth}{!}
{
{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{c|cc}
\hline
\toprule
\normalfont{ } 
\multirow{2}{*}{Model} & \multicolumn{2}{c}{SIDD~\cite{abdelhamed2018high}} \\
% \hline
 & PSNR & SSIM \\
\hline
MPRNet~\cite{zamir2021multi} & 17.48 & 0.4720 \\
TransWeather~\cite{valanarasu2022transweather} & 17.34 & 0.4934 \\
NAFNet~\cite{chen2022simple} & 17.67 & 0.4870 \\
WeatherDiffusion~\cite{ozdenizci2023weatherdiffusion} & 6.56 & 0.0050 \\
FocalNet~\cite{cui2023focal} & 17.87 &  0.5007 \\


\textbf{MetaWeather} & 18.63 & 0.4740 \\
\bottomrule
\end{tabular}
}
}

% \vspace{-11pt}
\label{tab:supp_sidd}
\end{table*}

==> table/supp_support_set.tex <==

\begin{table*}[ht!]
\centering
\caption{Ablation study on various shots. The \textbf{best} results for each number of shots are highlighted.}
\def\arraystretch{1.25}
\resizebox{1.0\columnwidth}{!}{
{\small
\setlength{\tabcolsep}{2.35pt}
\begin{tabular}{c|c|cc|cc|cc|cc|cc||cc}
\hline
\toprule
\normalfont{ } 
\multirow{2}{*}{\# of shots} & \multirow{2}{*}{Model} & \multicolumn{2}{c|}{$\text{R+S}$} & \multicolumn{2}{c|}{$\text{R+H}_\text{L}$} & \multicolumn{2}{c|}{$\text{R+H}_\text{H}$} & \multicolumn{2}{c|}{R+D+H$_\text{M}$} & \multicolumn{2}{c||}{R+D+S+H$_\text{M}$}  & \multicolumn{2}{c}{Average}\\
% \hline
& & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\
\hline
\multirow{9}{*}{1}&MPRNet~\cite{zamir2021multi} & 25.96 & 0.8397 & 22.75 & 0.8572 & 18.02 & 0.7291 & 18.70 & 0.7391 & 18.57 & 0.6682 & 20.80 & 0.7667\\
&TransWeather~\cite{valanarasu2022transweather} & 24.27 & 0.7869 & 22.89 & 0.8394 & 18.20 & 0.7348 & 19.63 & 0.7365 & 19.45 & 0.6412 & 20.89 & 0.7478\\
&AirNet~\cite{li2022all}  & 25.34 & 0.7631 & 21.25 & 0.7704 & 17.00 & 0.6738 & 17.50 & 0.6404 & 18.42 & 0.5908 & 19.90 & 0.6877\\
&MAXIM~\cite{tu2022maxim} & 26.44 & 0.8086 & 21.11 & 0.8298 & 17.51 & 0.7054 & 15.49 & 0.6519 & 17.78 & 0.6270 & 19.67 & 0.7245\\
&Restormer~\cite{zamir2022restormer} & 26.39 & \underline{0.8501} & 22.81 & 0.8450 & 15.43 & 0.6733 & 19.92 & 0.7602 & 16.75 & 0.6713 & 20.26 & 0.7600\\
&NAFNet~\cite{chen2022simple} & \underline{26.82} & 0.8393 & 22.40 & 0.8508 & 17.78 & 0.7207 & 19.87 & 0.7602 & 16.95 & 0.6609 & 20.76 & 0.7664\\
&WeatherDiffusion~\cite{ozdenizci2023weatherdiffusion} & 25.54 & 0.8431 & 23.17 & 0.8077 & \underline{21.17} & \underline{0.7720} & \underline{20.64} & 0.7623 & \underline{20.80} & \textbf{0.7735} & \underline{22.26} & \underline{0.7917}\\
&FocalNet~\cite{cui2023focal} & 25.85 & 0.8164 & \underline{23.47} & \underline{0.8604} & 19.28 & 0.7566 & 20.46 & \underline{0.7663} & 18.57 & 0.6707 & 21.53 & 0.7741\\

&\textbf{MetaWeather} & \textbf{27.88} & \textbf{0.8574} & \textbf{25.85} & \textbf{0.8790} & \textbf{22.02} & \textbf{0.8137} & \textbf{23.24} & \textbf{0.8142} & \textbf{22.42} & \underline{0.7575} & \textbf{24.28} & \textbf{0.8244}\\

\hline
% \multirow{6}{*}{\shortstack{ Few-shot\\ Adaptation}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\multirow{9}{*}{2}&MPRNet~\cite{zamir2021multi} & 27.98 & 0.8655 & 24.70 & 0.8849 & 20.44 & 0.8008 & 19.81 & 0.7725 & 20.94 & 0.7390 & 22.77 & 0.8125\\
&TransWeather~\cite{valanarasu2022transweather} & 25.82 & 0.8056 & 24.68 & 0.8484 & 21.48 & 0.7770 & 21.71 & 0.7569 & 20.72 & 0.6900 & 22.88 & 0.7756\\
&AirNet~\cite{li2022all}  & 26.63 & 0.8206 & 23.43 & 0.8535 & 17.35 & 0.7260 & 18.06 & 0.7130 & 17.97 & 0.6493 & 20.69 & 0.7525\\
&MAXIM~\cite{tu2022maxim} & 26.44 & 0.8086 & 21.11 & 0.8298 & 17.51 & 0.7054 & 15.49 & 0.6519 & 17.78 & 0.6270 & 19.67 & 0.7245\\
&Restormer~\cite{zamir2022restormer} & 27.73 & \textbf{0.8773} & 25.14 & 0.8791 & 20.75 & 0.7905 & 21.21 & 0.7871 & 18.52 & 0.7311 & 22.67 & 0.8130\\
&NAFNet~\cite{chen2022simple} & 26.45 & 0.8428 & 24.96 & 0.8724 & 20.91 & 0.7808 & 21.29 & 0.7751 & 19.52 & 0.7001 & 22.63 & 0.7942\\
&WeatherDiffusion~\cite{ozdenizci2023weatherdiffusion} & 25.54 & 0.8432 & 23.12 & 0.8066 & 21.17 & 0.7724 & 20.70 & 0.7646 & 20.81 & 0.7734 & 22.27 & 0.7920\\
&FocalNet~\cite{cui2023focal} & 26.58 & 0.8358 & 24.51 & 0.8636 & 20.16 & 0.7677 & 20.62 & 0.7599 & 18.79 & 0.6909 & 22.13 & 0.7836\\

&\textbf{MetaWeather} & \textbf{28.54} & \underline{0.8728} & \textbf{25.77} & \textbf{0.8876} & \textbf{22.58} & \textbf{0.8281} & \textbf{22.80} & \textbf{0.8188} & \textbf{22.16} & \textbf{0.7775} & \textbf{24.37} & \textbf{0.8370}\\

\hline


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{9}{*}{4}&MPRNet~\cite{zamir2021multi} & -\\
&TransWeather~\cite{valanarasu2022transweather} & -\\
&AirNet~\cite{li2022all}  & -\\
&MAXIM~\cite{tu2022maxim} & -\\
&Restormer~\cite{zamir2022restormer} & -\\
&NAFNet~\cite{chen2022simple} & -\\
&WeatherDiffusion~\cite{ozdenizci2023weatherdiffusion} & 25.49 & 0.8428 & 23.18 & 0.8077 & 21.19 & 0.7720 & 20.60 & 0.7616 & 20.80 & 0.7743 & 22.25 & 0.7917\\
&FocalNet~\cite{cui2023focal} & 26.46 & 0.8154 & 24.35 & 0.8719 & 19.76 & 0.7757 & 20.93 & 0.7815 & 20.76 & 0.7097 & 22.45 & 0.7908\\

&\textbf{MetaWeather} & 28.62 & 0.8780 & 26.17 & 0.8928 & 23.40 & 0.8422 & 23.59 & 0.8349 & 22.99 & 0.7937 & 24.95 & 0.8483\\


\bottomrule
\end{tabular}
}
}
% \caption{Quantitative evaluation on RealMCVSR dataset. † indicates that results are obtained from~\cite{lee2022reference}. - indicates that the information is not provided in the paper. Best results are \textbf{highlighted} and second-best results are {underlined}.}
\label{tab:sup_shot}
\end{table*}

